The Web Can Be Your Oyster for Improving Large Language Models

Large language models (LLMs) encode a large amount of world knowledge. However, as such knowledge is frozen at the time of model training, the models become static and limited by the training data at that time. In order to further improve the capacity of LLMs for knowledge-intensive tasks, we consider augmenting LLMs with the large-scale web using search engine. Unlike previous augmentation sources (e.g., Wikipedia data dump), the web provides broader, more comprehensive and constantly updated information. In this paper, we present a web-augmented LLM UNIWEB, which is trained over 16 knowledge-intensive tasks in a unified text-to-text format. Instead of simply using the retrieved contents from web, our approach has made two major improvements. Firstly, we propose an adaptive search engine assisted learning method that can self-evaluate the confidence level of LLM's predictions, and adaptively determine when to refer to the web for more data, which can avoid useless or noisy augmentation from web. Secondly, we design a pretraining task, i.e., continual knowledge learning, based on salient spans prediction, to reduce the discrepancy between the encoded and retrieved knowledge. Experiments on a wide range of knowledge-intensive tasks show that our model significantly outperforms previous retrieval-augmented methods.

==> sec-ethic.tex <==
\section{Ethical Concerns}

Current NAR text generation technology achieves faster inference speed but suffer from several issues like multi-modality, lack of accuracy to the input, commonsense issues etc., which makes their online real-time deployment difficult. \textsc{Elmer} is an effort at rectifying some of these issues, with a focus of modeling the semantic dependency between target tokens to improve NAR generation quality. However, compared to AR models, \textsc{Elmer} outputs continue to mix multiple candidates and repeat words at times. This should be strongly considered before any direct deployment of real-world systems. 

On the other hand, text generation technology may be potentially misused for harmful applications. When deploying \textsc{Elmer} to online real-time platforms, the high-quality text generated by our work also makes it difficult to distinguish synthetic text from human-written text, such as fake news and stories.  It is somewhat difficult to anticipate the harmful usages of our method since they often involve repurposing our model in a totally different setting or for an unexpected purpose than we planned. To alleviate this problem, we can ask for help from classic security risk assessment frameworks such as detecting threats.



